Labeling Comic Mischief Content in Online Videos with a Multimodal Hierarchical-Cross-Attention Model

We address the challenge of detecting questionable content in online media, specifically the subcategory of comic mischief. This type of content combines elements such as violence, adult content, or sarcasm with humor, making it difficult to detect. Employing a multimodal approach is vital to capture the subtle details inherent in comic mischief content. To tackle this problem, we propose a novel end-to-end multimodal system for the task of comic mischief detection. As part of this contribution, we release a novel dataset for the targeted task consisting of three modalities: video, text (video captions and subtitles), and audio. We also design a HIerarchical Cross-attention model with CAPtions (HICCAP) to capture the intricate relationships among these modalities. The results show that the proposed approach makes a significant improvement over robust baselines and state-of-the-art models for comic mischief detection and its type classification. This emphasizes the potential of our system to empower users, to make informed decisions about the online content they choose to see. In addition, we conduct experiments on the UCF101, HMDB51, and XD-Violence datasets, comparing our model against other state-of-the-art approaches showcasing the outstanding performance of our proposed model in various scenarios.

==> abstract.tex <==
%In this paper, we address the challenge of detecting questionable content in online media, specifically the subcategory of comic mischief. This type of content mixes questionable content such as violence, adult content, or sarcasm with humor, making it difficult to detect. To tackle this problem, we propose a novel end-to-end multimodal system for the task of comic mischief detection. A novel dataset for the approached task is released as part of this contribution, it consists of three modalities: video, text (video caption and subtitle), and audio. 
%To tackle this issue, the HIerarchical Cross attention model with CAPtions (HICCAP), is designed to capture the intricate relationships among these modalities.  We pretrain HICCAP using HowTo100M and Violent Scenes datasets and fine-tune with our own dataset. Also, we use the contrastive learning technique to jointly learn language, audio, and video representations to further improve the performance of the model using the kinetics-400 dataset. Our proposed approach demonstrates significant improvement over solid baselines and state-of-the-art models on comparable topics, highlighting the potential of our system in protecting users, especially children, from harmful online content\footnote{The dataset and code associated with this contribution will be released upon acceptance for publication.}.

We address the challenge of detecting questionable content in online media, specifically the subcategory of comic mischief. This type of content combines elements such as violence, adult content, or sarcasm with humor, making it difficult to detect. %When recognizing the inherent multifaceted nature of such content, the multimodal aspect becomes crucial. Combining different modalities offers a comprehensive perspective, capturing nuances that single-modality approaches might miss. This combination answers the pivotal question: why is it vital to fuse these modalities for this particular task? 
Employing a multimodal approach is vital to capture the subtle details inherent in comic mischief content.
To tackle this problem, we propose a novel end-to-end multimodal system for the task of comic mischief detection. 
As part of this contribution, we release a novel dataset for the targeted task consisting of three modalities: video, text (video captions and subtitles), and audio. We also design a HIerarchical Cross-attention model with CAPtions (HICCAP) to capture the intricate relationships among these modalities. 
%We pretrain HICCAP using the HowTo100M and Kinetics-400 datasets and fine-tune it with our own dataset. 
%Besides, multimodal matching and contrastive learning tasks were adopted for pretraining the model aiming to jointly learn the language, audio, and video representations.
The initial results show that the proposed approach makes a significant improvement over robust baselines and state-of-the-art models for comic mischief detection and its type classification.
This emphasizes the potential of our system to empower users, to make informed decisions about the online content they choose to see.
%highlighting the potential of our system in protecting users, especially children, from harmful online content
%Furthermore, extensive experiments on standard benchmarks (UCF101, HMDB51, and XD-Violence) demonstrate that our approach is effective and can be generalized to different video recognition scenarios.
%In addition, we conduct experiments on the UCF101, HMDB51, and XD-Violence datasets, comparing our model against other state-of-the-art approaches showcasing the superiority of our proposed model in various scenarios.
In addition, we conduct experiments on the UCF101, HMDB51, and XD-Violence datasets, comparing our model against other state-of-the-art approaches showcasing the outstanding performance of our proposed model in various scenarios.

\footnote{https://github.com/RiTUAL-UH/Comic-Mischief-Prediction}
%In this paper, we address the challenge of detecting questionable content in online media, specifically within the subcategory of comic mischief. This unique form of content artfully blends elements like violence, adult themes, and sarcasm with humor, rendering its detection quite challenging. Recognizing the inherent multifaceted nature of such content, the multimodal aspect becomes crucial. Combining different modalities offers a comprehensive perspective, capturing nuances that single-modality approaches might miss. This combination answers the pivotal question: why is it vital to fuse these modalities for this particular task? To this end, we introduce a novel end-to-end multimodal system dedicated to comic mischief detection. Our contribution also encompasses the release of a distinct dataset tailored to this task, amalgamating three modalities: video, text (video captions and subtitles), and audio. In designing our detection solution, we introduce the HIerarchical Cross attention model with CAPtions (HICCAP), crafted to discern the complex interrelationships spanning these modalities. Preliminary training of HICCAP leverages the HowTo100M, and Kinetics-400 datasets, followed by fine-tuning using our bespoke dataset. Our methodology incorporates multimodal matching and contrastive learning during pretraining to synergistically develop language, audio, and video representations. The results are compelling. Our approach not only outpaces robust baselines but also eclipses state-of-the-art models. Such efficacy underscores our system's potential in safeguarding users, particularly young ones, from detrimental online content\footnote{Upon paper acceptance, the associated dataset and code will be publicly released.}



==> discussion.tex <==
\vspace{-0.1cm}
The model incorrectly predicted 256 instances, including 94 instances of comic mischief and 162 instances of the "none" group. Of the 94 incorrectly classified comic mischief instances, 87 were single-category (e.g., only sarcasm) out of a total of 344 single-category instances. Only 7 videos with multiple categories were incorrectly predicted. Hence, as expected, %This suggests that 
videos with more categories may be easier to detect as comic mischief. For the "none" group, 162 out of 267 were incorrectly predicted. This could be due to videos containing mature or violent content that is not humorous, or a smaller number of "none" instances making it harder for the model to find a pattern.

We annotated videos for three modalities as previously stated and used our best model to predict the outcome of different modalities. When using binary HICCAP on the test set, we found cases that were predicted as non-comic mischief videos. From our observations, only one of the modalities contained comic mischief, while the rest contained none. Note that, we have 184 mono-modal examples out of 702 samples, 14 of which are active by video, and 170 are active by dialogue. Moreover, the 15 incorrectly classified cases have three modalities, 12 of which lack dialogue, and only three have dialogue. These observations suggest that dialogue is a powerful modality and that when it is active, the model is more accurate. But is it just about dialogue modality or does it depend on how models encode dialogue modality? To answer this question, we used the early fusion model and found that 52 out of 108 incorrectly classified instances in the comic mischief class were mono-modal samples that dialogue is the active modality. On the other hand, using the HICCAP model which employs a hierarchical cross-attention paradigm, we obtained better results that demonstrate its capability of superior encoding of modalities.

\vspace{-0.2cm}

==> result.tex <==

%Comparisons with Prior Works
\subsection{Evaluation with other Standard Benchamrks}
We evaluate the efficacy of our method on three multimodal datasets, created for activity recognition task UCF-101 \cite{soomro2012ucf101}, HMDB51 \cite{kuehne2011hmdb}, and XD-Violence for anomaly detection task \cite{wu2020not}. More details about architectures and datasets are provided in the supplementary materials.
To generate captions for these datasets, our approach drew inspiration from the prompt generation technique detailed in X-Clip \cite{ni2022expanding}. Here, the authors adapted the text encoder, initially trained in language-image models, by incorporating a video-specific prompting mechanism. In this technique, they utilize the video content features to improve the text prompting process. The idea behind it is that appropriate contextual information can improve recognition. 
%For caption generation of these datasets, we were inspired by the prompt generation technique proposed in X-Clip \cite{ni2022expanding}. In this method, thu authors employed the text encoder pretrained in the language-image models and expanded it with a video-specific prompting scheme. The key idea is to leverage video content information to enhance text prompting. The intuition behind this is that appropriate contextual information can help the recognition. 

\subsubsection{Result on UCF101}
Column 3 in Table \ref{ucf101-hmdb51-result} summarizes the performance comparison between the proposed method and other methods on the UCF101 dataset. In the presented table, our method outperforms the majority of previously established techniques in terms of top-1 accuracy. Notably, there is only one method, VideoMAE V2\cite{wang2023videomae}, with which our results do not surpass. However, it's crucial to highlight that even in this instance, our performance is comparable to this paper's. Importantly, our method achieves this with a more streamlined strategy and a model with significantly fewer parameters. This underscores the efficacy and efficiency of our approach, demonstrating that competitive outcomes can be realized without the need for complex systems or excessive model parameters.


\subsubsection{Result on HMDB51}

On the HMDB51 dataset, as shown in Column 4 of Table \ref{ucf101-hmdb51-result}, our approach continues to exhibit superior performance over almost all existing methods. There is just one method, VideoMAE V2\cite{wang2023videomae}, that marginally surpasses our results. It's worth noting that the rationale and context provided for our performance against other methods in the earlier discussion apply here as well.

\begin{table}[h!]
\caption{Comparison with the state-of-the-art methods on UCF101 and HMDB51.}
\vspace{-0.2cm}
\centering
\scalebox{0.7}{
\begin{tabular}{|l|c|c|c|}
    \hline
    Method & Modality & UCF101 & HMDB51 \\
    \hline
    OPN \cite{lee2017unsupervised}                    & V     & 59.6 & 23.8 \\\hline
    VCOP \cite{xu2019self}                            & V     & 72.4 & 30.9 \\\hline
    SpeedNet \cite{benaim2020speednet}& V     & 81.1 & 48.8 \\\hline
    VTHCL \cite{yang2020video}& V     & 82.1 & 49.2 \\\hline
    Pace \cite{wang2020self}& V     & 77.1 & 36.6 \\\hline
    MemDPC \cite{han2020memory}& V     & 86.1 & 54.5 \\\hline
    CoCLR \cite{han2020self}& V     & 87.9 & 54.6 \\\hline
    RSPNet \cite{chen2021rspnet}& V     & 93.7 & 64.7 \\\hline
    VideoMoCo \cite{pan2021videomoco}& V     & 78.7 & 49.2 \\\hline
    Vi2CLR \cite{diba2021vi2clr}& V     & 89.1 & 55.7 \\\hline
    CVRL \cite{qian2021spatiotemporal}& V     & 94.4 & 70.6 \\\hline
    CORPf \cite{hu2021contrast}& V     & 93.5 & 68.0 \\\hline
    %$\rho$SimCLR$_{\rho=2}$ \cite{feichtenhofer2021large}& V     & 88.9 & N/A \\\hline
    %$\rho$SwAV$_{\rho=2}$ \cite{feichtenhofer2021large}& V     & 87.3 & N/A \\\hline
    %$\rho$MoCo$_{\rho=2}$ \cite{feichtenhofer2021large}& V     & 91.0 & N/A \\\hline
    %$\rho$BYOL$_{\rho=4}$ \cite{feichtenhofer2021large}& V     & 94.2 & 72.1 \\\hline
    MIL-NCE \cite{miech2020end}& T+V   & 91.3 & 61.0 \\\hline
    MMV \cite{alayrac2020self}& T+A+V & 92.5 & 69.6 \\\hline
    CPD \cite{li2020learning}& T+V   & 92.8 & 63.8 \\\hline
    ELO \cite{piergiovanni2020evolving}& A+V   & 93.8 & 67.4 \\\hline
    XDC \cite{alwassel2020self}& A+V   & 94.2 & 67.1 \\\hline
    GDT \cite{patrick2020multi}& A+V   & 95.2 & 72.8 \\\hline
    VideoMAE V1\cite{tong2022videomae}& V     & 96.1 & 73.3 \\\hline
    VideoMAE V2\cite{wang2023videomae}& V     & 99.6 & 88.1 \\\hline
    Ours & T+A+V & 98.87 & 76.64   \\\hline
\end{tabular}
}
%\vspace{-0.15cm}
\label{ucf101-hmdb51-result}
\vspace{-0.05cm}
\end{table}

\subsubsection{Result on XD-Violence}
In this section, we applied our method to the XD-Violence dataset. Due to the lack of access to part of the provided vector features, we regenerate the I3D and VGGish features using the provided training and test videos. Similar to \cite{wu2021learning}, we use the frame-level precision-recall curve (PRC) and corresponding area under the curve (average precision, AP) and report the results in Table \ref{XD-result}. As shown in this table, our method achieves the new state-of-the-art performance of 92.17\% AP and gains clear improvements when compared with previous SOTA methods in terms of AP.


\begin{table}[h!]
\caption{Comparison with the state-of-the-art methods on XD-Violence. ‘V’, ‘A’, and ‘T’ denote video, audio, and text, respectively.}
\vspace{-0.2cm}
\centering
\scalebox{0.75}{
\begin{tabular}{|l|c|c|}
    \hline
    Method & Modality & AP (\%) \\
    \hline
    SVM Baseline                 & V     & 50.78  \\\hline
    OCSVM \cite{scholkopf1999support}  & V     & 27.25  \\\hline
    Hasan et al. \cite{hasan2016learning}     & V     & 30.77  \\\hline
    Wu et al. \cite{wu2021learning}        & V     & 75.9  \\\hline
    Contrastive Att. \cite{chang2021contrastive}  & V     & 76.9  \\\hline
    Yu et al. \cite{tian2021weakly}        & V     & 77.81  \\\hline
    AVVD \cite{wu2022weakly}        & V     & 78.10  \\\hline
    NG-MIL \cite{park2023normality}     & V     & 78.51  \\\hline
    MSL \cite{li2022self}            & V     & 78.59  \\\hline
    MGFN \cite{chen2023mgfn}          & V     & 80.11  \\\hline
    SR3 \cite{wu2022self}            & V     & 80.26  \\\hline
    CU-Net \cite{zhang2023exploiting}   & A+V     & 81.43  \\\hline
    Pang et al. \cite{pang2021violence}      & A+V     & 81.69  \\\hline
    DMU \cite{zhou2023dual}          & A+V     & 81.77   \\\hline
    CLIP-TSA \cite{joo2023clip}           & V     & 82.19  \\\hline
    MACIL-SD \cite{yu2022modality}        & A+V     & 83.4  \\\hline
    DDl \cite{pu2022audio}           & A+V     & 83.54  \\\hline
    Song et al. \cite{fan2023weakly}         & A+V   & 84.23  \\\hline
    VadCLIP \cite{wu2023vadclip} & V+T   & 84.51  \\\hline
    Ours & T+A+V   & 92.17  \\\hline
\end{tabular}
}
%\vspace{-0.15cm}
\label{XD-result}
\vspace{-0.05cm}
\end{table}


\subsection{Error Analysis}
The model incorrectly predicted 22 instances, including 11 instances of comic mischief and 11 instances of the "none" group. Of the 11 incorrectly classified comic mischief instances, 10 were single-category (e.g., only sarcasm) out of a total of 61 single-category instances. Only one video with multiple categories was also incorrectly predicted. Hence, as expected, %This suggests that 
videos with more categories may be easier to detect as comic mischief. For the "none" group, 11 out of 31 were incorrectly predicted. This could be due to videos containing mature or violent content that is not humorous, or a smaller number of "none" instances making it harder for the model to find a pattern.

%The model fails to predict 22 instances correctly (11 instances from comic mischief, 11 instances from the ``none'' group). From the 11 incorrectly classified comic mischief instances, 10 cases are single-category  (e.g., only include sarcasm), while in total we have 61 single-category instances. Only, one video with more than one category is also predicted incorrectly out of 22. Thus, we can hypothesize that the more categories (comic mischief categories) the video has, it is easier to be detected as comic mischief. From the group ``none'', 11 out of 31 are predicted incorrectly, we have two assumptions: first, some videos include mature or violent content, but not in a humorous context; and second, we have a smaller number of none instances, making it more difficult for the model to find a  pattern.



We annotated videos for three modalities as previously stated and used our best model to predict the outcome of different modalities. When using binary HICCAP on the test set, we found cases that were predicted as non-comic mischief videos. From our observations, we found that only one of the modalities contained comic mischief, while the rest contained none. Also, we have 26 mono-modal examples out of 113 samples, two of which are active by video, and 24 are dialogue. Moreover, the five incorrectly classified cases have three modalities, four of which lack dialogue, and only one has dialogue. These observations suggest that dialogue is a powerful modality and that when it is active, the model is more accurate. But is it just about dialogue modality or does it depend on how models encode dialogue modality? To answer this question, we used the early fusion model and found that 15 out of 50 incorrectly classified instances in the comic mischief class were mono-modal samples, all of which had dialogue as the active modality. On the other hand, using the HICCAP model which employs a hierarchical cross-attention paradigm, we obtained better results that demonstrate its capability of superior encoding of modalities.



